CommanderSong: A Systematic Approach for Practical Adversarial Voice Recognition

The popularity of ASR (automatic speech recognition) systems, like Google Voice, Cortana, brings in security concerns, as demonstrated by recent attacks. The impacts of such threats, however, are less clear, since they are either less stealthy (producing noise-like voice commands) or requiring the physical presence of an attack device (using ultrasound). In this paper, we demonstrate that not only are more practical and surreptitious attacks feasible but they can even be automatically constructed. Specifically, we find that the voice commands can be stealthily embedded into songs, which, when played, can effectively control the target system through ASR without being noticed. For this purpose, we developed novel techniques that address a key technical challenge: integrating the commands into a song in a way that can be effectively recognized by ASR through the air, in the presence of background noise, while not being detected by a human listener. Our research shows that this can be done automatically against real world ASR applications. We also demonstrate that such CommanderSongs can be spread through Internet (e.g., YouTube) and radio, potentially affecting millions of ASR users. We further present a new mitigation technique that controls this threat.

==> equations1.tex <==
Figure~\ref{overflow} demonstrates the details of our attack approach. We use Kaldi to decode the song audio $x(t)$ and command audio $y(t)$ separately. By analyzing the decoding procedures, we can get the output of DNN matrix $\textbf{A}$ of the song audio (Step \textcircled{1} in Figure~\ref{overflow}) and the transition-ids sequence of the command audio (Step \textcircled{4} in Figure~\ref{overflow}). 

The DNN's output $A$ is a matrix containing the probability of each pdf-id at each frame. Suppose there are $n$ frames and $k$ pdf-ids, let $a_{i,j}$ ($1 \leq i\leq n, 1 \leq j \leq k$) be the element at the $i$th row and $j$th column in $A$, then $a_{i,j}$ represents the probability of pdf-id $j$ at frame $i$. For each frame, we calculate the most likely pdf-id as the one with the highest probability in that frame. That is,
\begin{equation*}
	m_i = \arg\max_{j}a_{i,j}.
\end{equation*}
Let $\mathbf{m} = (m_1, m_2, \dots, m_n)$. $\mathbf{m}$ represents a sequence of most likely pdf-ids of the original song audio $x(t)$. For simplification, we use $g$ to represent the function that takes the original wave as input and outputs a sequence of most likely pdf-ids based on DNN's predictions. That is,
\begin{equation*}
	g(x(t)) = \mathbf{m}.
\end{equation*}

At shown in Step~\textcircled{5} in Figure~\ref{overflow}, we can extract a sequence of pdf-id of the command $\mathbf{b} = (b_1, b_2, \dots, b_n)$, where $b_i$ ($1\leq i \leq n$) represents the pdf-id of the command at frame $i$. To have the original song decoded as the command, we need to identify the minimum modification $\delta(t)$ on $x(t)$ so that $\mathbf{m}$ is close to $\mathbf{b}$. Specifically, we minimize the L1 distance between $\mathbf{m}$ and $\mathbf{b}$.

Based on these observations we construct the following objective function:
\begin{equation} \label{eq:obj}
	\arg\min_{\delta(t)} \quad \lVert g\left(x(t) + \delta(t)\right) - \mathbf{b} \rVert_1.
\end{equation}
To ensure that the modified audio do not deviate too much from the original ones, we choose an upper bound $l$ for the L1 norm of the modifications and optimize the objective function Eq(~\ref{eq:obj}) under the constraint that $\left|\delta(t)\right|\leq l$. 

Finally, we use gradient descent~\cite{papernot2016cleverhans}, an iterative optimization algorithm to find the local minimum of a function, to solve the objective function. Given an initial point, gradient descent follows the direction which reduces the value of the function most quickly. By repeating this process until the value starts to increase, the algorithm is able to find a local minimum value. In particular, based on our objective function, we revise the song $x(t)$ into $x'(t) = x(t) + \delta(t)$ with the aim of making most likely pdf-ids $g\left(x'(t)\right) = \mathbf{b}$. Therefore, the crafted audio $x'(t)$ can be decoded as the desired command text. 

To further preserve the fidelity of the original song, one method is to minimize the time duration of the revision. Typically, once the command audio is generated by a text-to-speech engine, all the phonemes are determined, so as to the transition-id sequence and $\mathbf{b}$. However, the speech speed also determines the number of frames, and the number of transition-ids, for a phoneme. Intuitively, slow speech always produces repeated frames, or transition-ids, in a phoneme. Typically human needs six or more frames to realize a phoneme, but most speech recognition systems only need three to four frames to interpreted a phoneme. Hence, to introduce the minimal revision to the original song, we can analyze $\mathbf{b}$, reduce the number of repeated frames in each phoneme, and obtain a shorter $\mathbf{b}'=(b_1, b_2, \dots, b_q)$, where $q<n$.
